Compressing Recurrent Neural Networks with Tensor Ring for Action Recognition

Recurrent Neural Networks (RNNs) and their variants, such as Long-Short Term Memory (LSTM) networks, and Gated Recurrent Unit (GRU) networks, have achieved promising performance in sequential data modeling. The hidden layers in RNNs can be regarded as the memory units, which are helpful in storing information in sequential contexts. However, when dealing with high dimensional input data, such as video and text, the input-to-hidden linear transformation in RNNs brings high memory usage and huge computational cost. This makes the training of RNNs unscalable and difficult. To address this challenge, we propose a novel compact LSTM model, named as TR-LSTM, by utilizing the low-rank tensor ring decomposition (TRD) to reformulate the input-to-hidden transformation. Compared with other tensor decomposition methods, TR-LSTM is more stable. In addition, TR-LSTM can complete an end-to-end training and also provide a fundamental building block for RNNs in handling large input data. Experiments on real-world action recognition datasets have demonstrated the promising performance of the proposed TR-LSTM compared with the tensor train LSTM and other state-of-the-art competitors.

==> ref_backup.tex <==
@article{rumelhart1988learning,
  title={Learning representations by back-propagating errors},
  author={Rumelhart, David E and Hinton, Geoffrey E and Williams, Ronald J},
  journal={Cognitive modeling},
  volume={5},
  number={3},
  pages={1},
  year={1988}
}

@inproceedings{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
  booktitle={Advances in neural information processing systems},
  pages={3104--3112},
  year={2014}
}

@article{5_tucker_FC_CONV,
  author    = {Yong{-}Deok Kim and
               Eunhyeok Park and
               Sungjoo Yoo and
               Taelim Choi and
               Lu Yang and
               Dongjun Shin},
  title     = {Compression of Deep Convolutional Neural Networks for Fast and Low
               Power Mobile Applications},
  journal   = {CoRR},
  volume    = {abs/1511.06530},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.06530},
  archivePrefix = {arXiv},
  eprint    = {1511.06530},
  timestamp = {Mon, 13 Aug 2018 16:49:06 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/KimPYCYS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Ye_2018_CVPR,
author = {Ye, Jinmian and Wang, Linnan and Li, Guangxi and Chen, Di and Zhe, Shandian and Chu, Xinqi and Xu, Zenglin},
title = {Learning Compact Recurrent Neural Networks With Block-Term Tensor Decomposition},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@inproceedings{DBLP:conf/nips/NovikovPOV15,
  author    = {Alexander Novikov and
               Dmitry Podoprikhin and
               Anton Osokin and
               Dmitry P. Vetrov},
  editor    = {Corinna Cortes and
               Neil D. Lawrence and
               Daniel D. Lee and
               Masashi Sugiyama and
               Roman Garnett},
  title     = {Tensorizing Neural Networks},
  booktitle = {Advances in Neural Information Processing Systems 28: Annual Conference
               on Neural Information Processing Systems 2015, December 7-12, 2015,
               Montreal, Quebec, Canada},
  pages     = {442--450},
  year      = {2015},
  url       = {http://papers.nips.cc/paper/5787-tensorizing-neural-networks},
  timestamp = {Fri, 08 Apr 2016 19:32:53 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/nips/NovikovPOV15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Wang_2018_CVPR,
author = {Wang, Wenqi and Sun, Yifan and Eriksson, Brian and Wang, Wenlin and Aggarwal, Vaneet},
title = {Wide Compression: Tensor Ring Nets},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@article{DBLP:journals/corr/ZhaoZXZC16,
  author    = {Qibin Zhao and
               Guoxu Zhou and
               Shengli Xie and
               Liqing Zhang and
               Andrzej Cichocki},
  title     = {Tensor Ring Decomposition},
  journal   = {CoRR},
  volume    = {abs/1606.05535},
  year      = {2016},
  url       = {http://arxiv.org/abs/1606.05535},
  archivePrefix = {arXiv},
  eprint    = {1606.05535},
  timestamp = {Mon, 13 Aug 2018 16:46:59 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/ZhaoZXZC16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icml/YangKT17,
  author    = {Yinchong Yang and
               Denis Krompass and
               Volker Tresp},
  editor    = {Doina Precup and
               Yee Whye Teh},
  title     = {Tensor-Train Recurrent Neural Networks for Video Classification},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
  series    = {Proceedings of Machine Learning Research},
  volume    = {70},
  pages     = {3891--3900},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v70/yang17e.html},
  timestamp = {Wed, 16 Aug 2017 11:08:55 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/icml/YangKT17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/interspeech/XueLG13,
  author    = {Jian Xue and
               Jinyu Li and
               Yifan Gong},
  editor    = {Fr{\'{e}}d{\'{e}}ric Bimbot and
               Christophe Cerisara and
               C{\'{e}}cile Fougeron and
               Guillaume Gravier and
               Lori Lamel and
               Fran{\c{c}}ois Pellegrino and
               Pascal Perrier},
  title     = {Restructuring of deep neural network acoustic models with singular
               value decomposition},
  booktitle = {{INTERSPEECH} 2013, 14th Annual Conference of the International Speech
               Communication Association, Lyon, France, August 25-29, 2013},
  pages     = {2365--2369},
  publisher = {{ISCA}},
  year      = {2013},
  url       = {http://www.isca-speech.org/archive/interspeech\_2013/i13\_2365.html},
  timestamp = {Mon, 27 Jan 2014 20:38:49 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/interspeech/XueLG13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{
polino2018model,
title={Model compression via distillation and quantization},
author={Antonio Polino and Razvan Pascanu and Dan Alistarh},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=S1XolQbRW},
}

@article{DBLP:journals/corr/HintonVD15,
  author    = {Geoffrey E. Hinton and
               Oriol Vinyals and
               Jeffrey Dean},
  title     = {Distilling the Knowledge in a Neural Network},
  journal   = {CoRR},
  volume    = {abs/1503.02531},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.02531},
  archivePrefix = {arXiv},
  eprint    = {1503.02531},
  timestamp = {Mon, 13 Aug 2018 16:48:36 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HintonVD15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/LebedevGROL14,
  author    = {Vadim Lebedev and
               Yaroslav Ganin and
               Maksim Rakhuba and
               Ivan V. Oseledets and
               Victor S. Lempitsky},
  title     = {Speeding-up Convolutional Neural Networks Using Fine-tuned CP-Decomposition},
  journal   = {CoRR},
  volume    = {abs/1412.6553},
  year      = {2014},
  url       = {http://arxiv.org/abs/1412.6553},
  archivePrefix = {arXiv},
  eprint    = {1412.6553},
  timestamp = {Mon, 13 Aug 2018 16:47:41 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/LebedevGROL14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@phdthesis{sifre2014rigid,
  title={Rigid-motion scattering for image classification},
  author={Sifre, Laurent and Mallat, St{\'e}phane},
  year={2014},
  school={Citeseer}
}

@article{DBLP:journals/corr/HowardZCKWWAA17,
  author    = {Andrew G. Howard and
               Menglong Zhu and
               Bo Chen and
               Dmitry Kalenichenko and
               Weijun Wang and
               Tobias Weyand and
               Marco Andreetto and
               Hartwig Adam},
  title     = {MobileNets: Efficient Convolutional Neural Networks for Mobile Vision
               Applications},
  journal   = {CoRR},
  volume    = {abs/1704.04861},
  year      = {2017},
  url       = {http://arxiv.org/abs/1704.04861},
  archivePrefix = {arXiv},
  eprint    = {1704.04861},
  timestamp = {Mon, 13 Aug 2018 16:46:35 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/HowardZCKWWAA17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

% panyu part
@inproceedings{DBLP:conf/cvpr/LiuLS09,
  author    = {Jingen Liu and
               Jiebo Luo and
               Mubarak Shah},
  title     = {Recognizing realistic actions from videos},
  booktitle = {2009 {IEEE} Computer Society Conference on Computer Vision and Pattern
               Recognition {(CVPR} 2009), 20-25 June 2009, Miami, Florida, {USA}},
  pages     = {1996--2003},
  publisher = {{IEEE} Computer Society},
  year      = {2009},
  url       = {https://doi.org/10.1109/CVPRW.2009.5206744},
  doi       = {10.1109/CVPRW.2009.5206744},
  timestamp = {Thu, 25 May 2017 00:41:27 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/LiuLS09},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/wacv/GammulleDSF17,
  author    = {Harshala Gammulle and
               Simon Denman and
               Sridha Sridharan and
               Clinton Fookes},
  title     = {Two Stream {LSTM:} {A} Deep Fusion Framework for Human Action Recognition},
  booktitle = {2017 {IEEE} Winter Conference on Applications of Computer Vision,
               {WACV} 2017, Santa Rosa, CA, USA, March 24-31, 2017},
  pages     = {177--186},
  publisher = {{IEEE}},
  year      = {2017},
  url       = {https://doi.org/10.1109/WACV.2017.27},
  doi       = {10.1109/WACV.2017.27},
  timestamp = {Tue, 16 May 2017 15:19:37 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/wacv/GammulleDSF17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/HasanR14,
  author    = {Mahmudul Hasan and
               Amit K. Roy{-}Chowdhury},
  title     = {Incremental Activity Modeling and Recognition in Streaming Videos},
  booktitle = {2014 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2014, Columbus, OH, USA, June 23-28, 2014},
  pages     = {796--803},
  publisher = {{IEEE} Computer Society},
  year      = {2014},
  url       = {https://doi.org/10.1109/CVPR.2014.107},
  doi       = {10.1109/CVPR.2014.107},
  timestamp = {Thu, 25 May 2017 00:41:16 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/HasanR14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/eccv/Ikizler-CinbisS10,
  author    = {Nazli Ikizler{-}Cinbis and
               Stan Sclaroff},
  editor    = {Kostas Daniilidis and
               Petros Maragos and
               Nikos Paragios},
  title     = {Object, Scene and Actions: Combining Multiple Features for Human Action
               Recognition},
  booktitle = {Computer Vision - {ECCV} 2010, 11th European Conference on Computer
               Vision, Heraklion, Crete, Greece, September 5-11, 2010, Proceedings,
               Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {6311},
  pages     = {494--507},
  publisher = {Springer},
  year      = {2010},
  url       = {https://doi.org/10.1007/978-3-642-15549-9\_36},
  doi       = {10.1007/978-3-642-15549-9\_36},
  timestamp = {Fri, 19 May 2017 01:25:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/Ikizler-CinbisS10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/WangKSL11,
  author    = {Heng Wang and
               Alexander Kl{\"{a}}ser and
               Cordelia Schmid and
               Cheng{-}Lin Liu},
  title     = {Action recognition by dense trajectories},
  booktitle = {The 24th {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2011, Colorado Springs, CO, USA, 20-25 June 2011},
  pages     = {3169--3176},
  publisher = {{IEEE} Computer Society},
  year      = {2011},
  url       = {https://doi.org/10.1109/CVPR.2011.5995407},
  doi       = {10.1109/CVPR.2011.5995407},
  timestamp = {Thu, 25 May 2017 00:41:26 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/WangKSL11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/SharmaKS15,
  author    = {Shikhar Sharma and
               Ryan Kiros and
               Ruslan Salakhutdinov},
  title     = {Action Recognition using Visual Attention},
  journal   = {CoRR},
  volume    = {abs/1511.04119},
  year      = {2015},
  url       = {http://arxiv.org/abs/1511.04119},
  archivePrefix = {arXiv},
  eprint    = {1511.04119},
  timestamp = {Mon, 13 Aug 2018 16:48:12 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/SharmaKS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pr/ChoLCO14,
  author    = {Jungchan Cho and
               Minsik Lee and
               Hyung Jin Chang and
               Songhwai Oh},
  title     = {Robust action recognition using local motion and group sparsity},
  journal   = {Pattern Recognition},
  volume    = {47},
  number    = {5},
  pages     = {1813--1825},
  year      = {2014},
  url       = {https://doi.org/10.1016/j.patcog.2013.12.004},
  doi       = {10.1016/j.patcog.2013.12.004},
  timestamp = {Thu, 18 May 2017 09:54:31 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/pr/ChoLCO14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/iccv/KuehneJGPS11,
  author    = {Hildegard Kuehne and
               Hueihan Jhuang and
               Est{\'{\i}}baliz Garrote and
               Tomaso A. Poggio and
               Thomas Serre},
  editor    = {Dimitris N. Metaxas and
               Long Quan and
               Alberto Sanfeliu and
               Luc J. Van Gool},
  title     = {{HMDB:} {A} large video database for human motion recognition},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2011, Barcelona,
               Spain, November 6-13, 2011},
  pages     = {2556--2563},
  publisher = {{IEEE} Computer Society},
  year      = {2011},
  url       = {https://doi.org/10.1109/ICCV.2011.6126543},
  doi       = {10.1109/ICCV.2011.6126543},
  timestamp = {Wed, 24 May 2017 08:31:07 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iccv/KuehneJGPS11},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/CaiWPQ14,
  author    = {Zhuowei Cai and
               Limin Wang and
               Xiaojiang Peng and
               Yu Qiao},
  title     = {Multi-view Super Vector for Action Recognition},
  booktitle = {2014 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2014, Columbus, OH, USA, June 23-28, 2014},
  pages     = {596--603},
  publisher = {{IEEE} Computer Society},
  year      = {2014},
  url       = {https://doi.org/10.1109/CVPR.2014.83},
  doi       = {10.1109/CVPR.2014.83},
  timestamp = {Thu, 25 May 2017 00:41:13 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/CaiWPQ14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/WangS13a,
  author    = {Heng Wang and
               Cordelia Schmid},
  title     = {Action Recognition with Improved Trajectories},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2013, Sydney,
               Australia, December 1-8, 2013},
  pages     = {3551--3558},
  publisher = {{IEEE} Computer Society},
  year      = {2013},
  url       = {https://doi.org/10.1109/ICCV.2013.441},
  doi       = {10.1109/ICCV.2013.441},
  timestamp = {Wed, 24 May 2017 08:31:06 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iccv/WangS13a},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/TranBFTP15,
  author    = {Du Tran and
               Lubomir D. Bourdev and
               Rob Fergus and
               Lorenzo Torresani and
               Manohar Paluri},
  title     = {Learning Spatiotemporal Features with 3D Convolutional Networks},
  booktitle = {2015 {IEEE} International Conference on Computer Vision, {ICCV} 2015,
               Santiago, Chile, December 7-13, 2015},
  pages     = {4489--4497},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/ICCV.2015.510},
  doi       = {10.1109/ICCV.2015.510},
  timestamp = {Wed, 24 May 2017 08:31:05 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iccv/TranBFTP15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/FeichtenhoferPZ16,
  author    = {Christoph Feichtenhofer and
               Axel Pinz and
               Andrew Zisserman},
  title     = {Convolutional Two-Stream Network Fusion for Video Action Recognition},
  booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
  pages     = {1933--1941},
  publisher = {{IEEE} Computer Society},
  year      = {2016},
  url       = {https://doi.org/10.1109/CVPR.2016.213},
  doi       = {10.1109/CVPR.2016.213},
  timestamp = {Thu, 25 May 2017 00:41:18 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/FeichtenhoferPZ16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/Wang0T15,
  author    = {Limin Wang and
               Yu Qiao and
               Xiaoou Tang},
  title     = {Action recognition with trajectory-pooled deep-convolutional descriptors},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {4305--4314},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7299059},
  doi       = {10.1109/CVPR.2015.7299059},
  timestamp = {Thu, 25 May 2017 00:41:23 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/Wang0T15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/CarreiraZ17,
  author    = {Jo{\~{a}}o Carreira and
               Andrew Zisserman},
  title     = {Quo Vadis, Action Recognition? {A} New Model and the Kinetics Dataset},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {4724--4733},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.502},
  doi       = {10.1109/CVPR.2017.502},
  timestamp = {Sun, 05 Aug 2018 18:05:12 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/CarreiraZ17},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/NiMYY15,
  author    = {Bingbing Ni and
               Pierre Moulin and
               Xiaokang Yang and
               Shuicheng Yan},
  title     = {Motion Part Regularization: Improving action recognition via trajectory
               group selection},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {3698--3706},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7298993},
  doi       = {10.1109/CVPR.2015.7298993},
  timestamp = {Thu, 25 May 2017 00:41:27 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/NiMYY15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/eccv/JiangDXLN12,
  author    = {Yu{-}Gang Jiang and
               Qi Dai and
               Xiangyang Xue and
               Wei Liu and
               Chong{-}Wah Ngo},
  editor    = {Andrew W. Fitzgibbon and
               Svetlana Lazebnik and
               Pietro Perona and
               Yoichi Sato and
               Cordelia Schmid},
  title     = {Trajectory-Based Modeling of Human Actions with Motion Reference Points},
  booktitle = {Computer Vision - {ECCV} 2012 - 12th European Conference on Computer
               Vision, Florence, Italy, October 7-13, 2012, Proceedings, Part {V}},
  series    = {Lecture Notes in Computer Science},
  volume    = {7576},
  pages     = {425--438},
  publisher = {Springer},
  year      = {2012},
  url       = {https://doi.org/10.1007/978-3-642-33715-4\_31},
  doi       = {10.1007/978-3-642-33715-4\_31},
  timestamp = {Fri, 02 Jun 2017 20:49:18 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/JiangDXLN12},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/JainJB13,
  author    = {Mihir Jain and
               Herve Jegou and
               Patrick Bouthemy},
  title     = {Better Exploiting Motion for Better Action Recognition},
  booktitle = {2013 {IEEE} Conference on Computer Vision and Pattern Recognition,
               Portland, OR, USA, June 23-28, 2013},
  pages     = {2555--2562},
  publisher = {{IEEE} Computer Society},
  year      = {2013},
  url       = {https://doi.org/10.1109/CVPR.2013.330},
  doi       = {10.1109/CVPR.2013.330},
  timestamp = {Thu, 25 May 2017 00:41:24 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/JainJB13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/ZhuWYZT13,
  author    = {Jun Zhu and
               Baoyuan Wang and
               Xiaokang Yang and
               Wenjun Zhang and
               Zhuowen Tu},
  title     = {Action Recognition with Actons},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2013, Sydney,
               Australia, December 1-8, 2013},
  pages     = {3559--3566},
  publisher = {{IEEE} Computer Society},
  year      = {2013},
  url       = {https://doi.org/10.1109/ICCV.2013.442},
  doi       = {10.1109/ICCV.2013.442},
  timestamp = {Wed, 24 May 2017 08:31:07 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iccv/ZhuWYZT13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/eccv/PengZQP14,
  author    = {Xiaojiang Peng and
               Changqing Zou and
               Yu Qiao and
               Qiang Peng},
  editor    = {David J. Fleet and
               Tom{\'{a}}s Pajdla and
               Bernt Schiele and
               Tinne Tuytelaars},
  title     = {Action Recognition with Stacked Fisher Vectors},
  booktitle = {Computer Vision - {ECCV} 2014 - 13th European Conference, Zurich,
               Switzerland, September 6-12, 2014, Proceedings, Part {V}},
  series    = {Lecture Notes in Computer Science},
  volume    = {8693},
  pages     = {581--595},
  publisher = {Springer},
  year      = {2014},
  url       = {https://doi.org/10.1007/978-3-319-10602-1\_38},
  doi       = {10.1007/978-3-319-10602-1\_38},
  timestamp = {Fri, 19 May 2017 01:25:57 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/eccv/PengZQP14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
% panyu part end

@article{DBLP:journals/siammax/SilvaL08,
  author    = {Vin de Silva and
               Lek{-}Heng Lim},
  title     = {Tensor Rank and the Ill-Posedness of the Best Low-Rank Approximation
               Problem},
  journal   = {{SIAM} J. Matrix Analysis Applications},
  volume    = {30},
  number    = {3},
  pages     = {1084--1127},
  year      = {2008},
  url       = {https://doi.org/10.1137/06066518X},
  doi       = {10.1137/06066518X},
  timestamp = {Fri, 26 May 2017 22:53:28 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/siammax/SilvaL08},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


%--------------------------
@article{XuYQ15tensor,
  author    = {Zenglin Xu and
               Feng Yan and
               Yuan (Alan) Qi},
  title     = {Bayesian Nonparametric Models for Multiway Data Analysis},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {37},
  number    = {2},
  pages     = {475--487},
  year      = {2015},
}

@article{liyycyx17tensor,
  author    = {Guangxi Li and
               Jinmian Ye and
               Haiqin Yang and
               Di Chen and
               Shuicheng Yan and
               Zenglin Xu},
  title     = {BT-Nets: Simplifying Deep Neural Networks via Block Term Decomposition},
  journal   = {CoRR},
  volume    = {abs/1712.05689},
  year      = {2017},
}


@inproceedings{XuYQ12icmltensor,
  author    = {Zenglin Xu and
               Feng Yan and
               Yuan (Alan) Qi},
  title     = {Infinite Tucker Decomposition: Nonparametric Bayesian Models for Multiway
               Data Analysis},
  booktitle = {Proceedings of the 29th International Conference on Machine Learning,
               {ICML} 2012, Edinburgh, Scotland, UK, June 26 - July 1, 2012},
  year      = {2012},
}

@inproceedings{denil2013predicting,
  title={Predicting parameters in deep learning},
  author={Denil, Misha and Shakibi, Babak and Dinh, Laurent and de Freitas, Nando and others},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2148--2156},
  year={2013}
}
@article{jaderberg2014speeding,
  title={Speeding up convolutional neural networks with low rank expansions},
  author={Jaderberg, Max and Vedaldi, Andrea and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1405.3866},
  year={2014}
}
@article{molchanov2016pruning,
  title={Pruning Convolutional Neural Networks for Resource Efficient Inference},
  author={Molchanov, Pavlo and Tyree, Stephen and Karras, Tero and Aila, Timo and Kautz, Jan},
  year={2016}
}

@inproceedings{lu2016learning,
  title={Learning compact recurrent neural networks},
  author={Lu, Zhiyun and Sindhwani, Vikas and Sainath, Tara N},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2016 IEEE International Conference on},
  pages={5960--5964},
  year={2016},
  organization={IEEE}
}
@inproceedings{prabhavalkar2016compression,
  title={On the compression of recurrent neural networks with an application to LVCSR acoustic modeling for embedded speech recognition},
  author={Prabhavalkar, Rohit and Alsharif, Ouais and Bruguier, Antoine and McGraw, Lan},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2016 IEEE International Conference on},
  pages={5970--5974},
  year={2016},
  organization={IEEE}
}







@article{hodosh2013framing,
  title={Framing image description as a ranking task: Data, models and evaluation metrics},
  author={Hodosh, Micah and Young, Peter and Hockenmaier, Julia},
  journal={Journal of Artificial Intelligence Research},
  volume={47},
  pages={853--899},
  year={2013}
}

@InProceedings{marszalek09,
    author = "Marcin Marsza{\l}ek and Ivan Laptev and Cordelia Schmid",
    title = "Actions in Context",
    booktitle = "IEEE Conference on Computer Vision \& Pattern Recognition",
    year = "2009"
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@article{chollet2015keras,
  title={Keras: Deep learning library for theano and tensorflow},
  author={Chollet, Fran{\c{c}}ois and others},
  journal={URL: https://keras. io/k},
  year={2015}
}

@article{abadi2016tensorflow,
  title={Tensorflow: Large-scale machine learning on heterogeneous distributed systems},
  author={Abadi, Mart{\'\i}n and Agarwal, Ashish and Barham, Paul and Brevdo, Eugene and Chen, Zhifeng and Citro, Craig and Corrado, Greg S and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and others},
  journal={arXiv preprint arXiv:1603.04467},
  year={2016}
}

@article{sorber2013optimization,
  title={Optimization-based algorithms for tensor decompositions: Canonical polyadic decomposition, decomposition in rank-(L\_r,L\_r,1) terms, and a new generalization},
  author={Sorber, Laurent and Van Barel, Marc and De Lathauwer, Lieven},
  journal={SIAM Journal on Optimization},
  volume={23},
  number={2},
  pages={695--720},
  year={2013},
  publisher={SIAM}
}

@article{carroll1970analysis,
  title={Analysis of individual differences in multidimensional scaling via an N-way generalization of “Eckart-Young” decomposition},
  author={Carroll, J Douglas and Chang, Jih-Jie},
  journal={Psychometrika},
  volume={35},
  number={3},
  pages={283--319},
  year={1970},
  publisher={Springer}
}

@article{tucker1966some,
  title={Some mathematical notes on three-mode factor analysis},
  author={Tucker, Ledyard R},
  journal={Psychometrika},
  volume={31},
  number={3},
  pages={279--311},
  year={1966},
  publisher={Springer}
}

@article{oseledets2011tensor,
  title={Tensor-train decomposition},
  author={Oseledets, Ivan V},
  journal={SIAM Journal on Scientific Computing},
  volume={33},
  number={5},
  pages={2295--2317},
  year={2011},
  publisher={SIAM}
}

@article{de2008decompositions2,
  title={Decompositions of a higher-order tensor in block terms—Part II: Definitions and uniqueness},
  author={De Lathauwer, Lieven},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={30},
  number={3},
  pages={1033--1066},
  year={2008},
  publisher={SIAM}
}

@article{de2008decompositions3,
  title={Decompositions of a higher-order tensor in block terms—Part III: Alternating least squares algorithms},
  author={De Lathauwer, Lieven and Nion, Dimitri},
  journal={SIAM journal on Matrix Analysis and Applications},
  volume={30},
  number={3},
  pages={1067--1083},
  year={2008},
  publisher={SIAM}
}

@article{werbos1990backpropagation,
  title={Backpropagation through time: what it does and how to do it},
  author={Werbos, Paul J},
  journal={Proceedings of the IEEE},
  volume={78},
  number={10},
  pages={1550--1560},
  year={1990},
  publisher={IEEE}
}

@article{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.1078},
  year={2014}
}

@inproceedings{sainath2013low,
  title={Low-rank matrix factorization for deep neural network training with high-dimensional output targets},
  author={Sainath, Tara N and Kingsbury, Brian and Sindhwani, Vikas and Arisoy, Ebru and Ramabhadran, Bhuvana},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2013 IEEE International Conference on},
  pages={6655--6659},
  year={2013},
  organization={IEEE}
}

@inproceedings{chen2015compressing,
  title={Compressing neural networks with the hashing trick},
  author={Chen, Wenlin and Wilson, James and Tyree, Stephen and Weinberger, Kilian and Chen, Yixin},
  booktitle={International Conference on Machine Learning},
  pages={2285--2294},
  year={2015}
}

@inproceedings{zeiler2014visualizing,
  title={Visualizing and understanding convolutional networks},
  author={Zeiler, Matthew D and Fergus, Rob},
  booktitle={European conference on computer vision},
  pages={818--833},
  year={2014},
  organization={Springer}
}

@article{han2015deep,
  title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
  author={Han, Song and Mao, Huizi and Dally, William J},
  journal={arXiv preprint arXiv:1510.00149},
  year={2015}
}


@article{DBLP:journals/corr/abs-1708-00185,
  author    = {Mingyuan Bai and
               Boyan Zhang and
               Junbin Gao},
  title     = {Tensorial Recurrent Neural Networks for Longitudinal Data Analysis},
  journal   = {CoRR},
  volume    = {abs/1708.00185},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.00185},
  archivePrefix = {arXiv},
  eprint    = {1708.00185},
  timestamp = {Mon, 13 Aug 2018 16:47:44 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1708-00185},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{elman1990finding,
  title={Finding structure in time},
  author={Elman, Jeffrey L},
  journal={Cognitive science},
  volume={14},
  number={2},
  pages={179--211},
  year={1990},
  publisher={Wiley Online Library}
}

@article{kolda2009tensor,
  title={Tensor decompositions and applications},
  author={Kolda, Tamara G and Bader, Brett W},
  journal={SIAM review},
  volume={51},
  number={3},
  pages={455--500},
  year={2009},
  publisher={SIAM}
}

@article{hochreiter1991untersuchungen,
  title={Untersuchungen zu dynamischen neuronalen Netzen},
  author={Hochreiter, Sepp},
  journal={Diploma, Technische Universit{\"a}t M{\"u}nchen},
  volume={91},
  year={1991}
}

@article{bengio1994learning,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Bengio, Yoshua and Simard, Patrice and Frasconi, Paolo},
  journal={IEEE transactions on neural networks},
  volume={5},
  number={2},
  pages={157--166},
  year={1994},
  publisher={IEEE}
}

@article{mikolov2012statistical,
  title={Statistical language models based on neural networks},
  author={Mikolov, Tom{\'a}{\v{s}}},
  journal={Presentation at Google, Mountain View, 2nd April},
  year={2012}
}

@inproceedings{pascanu2013difficulty,
  title={On the difficulty of training recurrent neural networks},
  author={Pascanu, Razvan and Mikolov, Tomas and Bengio, Yoshua},
  booktitle={International Conference on Machine Learning},
  pages={1310--1318},
  year={2013}
}

@inproceedings{jozefowicz2015empirical,
  title={An empirical exploration of recurrent network architectures},
  author={Jozefowicz, Rafal and Zaremba, Wojciech and Sutskever, Ilya},
  booktitle={Proceedings of the 32nd International Conference on Machine Learning (ICML-15)},
  pages={2342--2350},
  year={2015}
}


@article{gregor2015draw,
  title={DRAW: A recurrent neural network for image generation},
  author={Gregor, Karol and Danihelka, Ivo and Graves, Alex and Rezende, Danilo Jimenez and Wierstra, Daan},
  journal={arXiv preprint arXiv:1502.04623},
  year={2015}
}

@inproceedings{lin2014microsoft,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European conference on computer vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}

@inproceedings{vinyals2015show,
  title={Show and tell: A neural image caption generator},
  author={Vinyals, Oriol and Toshev, Alexander and Bengio, Samy and Erhan, Dumitru},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3156--3164},
  year={2015}
}

@article{lecun1995convolutional,
  title={Convolutional networks for images, speech, and time series},
  author={LeCun, Yann and Bengio, Yoshua and others},
  journal={The handbook of brain theory and neural networks},
  volume={3361},
  number={10},
  pages={1995},
  year={1995}
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@article{yunpeng2017sharing,
  title={Sharing Residual Units Through Collective Tensor Factorization in Deep Neural Networks},
  author={Yunpeng, Chen and Xiaojie, Jin and Bingyi, Kang and Jiashi, Feng and Shuicheng, Yan},
  journal={arXiv preprint arXiv:1703.02180},
  year={2017}
}


@inproceedings{liu2013spatial,
  title={Spatial-temporal motion information integration for action detection and recognition in non-static background},
  author={Liu, Dianting and Shyu, Mei-Ling and Zhao, Guiru},
  booktitle={Information Reuse and Integration (IRI), 2013 IEEE 14th International Conference on},
  pages={626--633},
  year={2013},
  organization={IEEE}
}

@article{lin2013network,
  title={Network in network},
  author={Lin, Min and Chen, Qiang and Yan, Shuicheng},
  journal={arXiv preprint arXiv:1312.4400},
  year={2013}
}


@article{cichocki2014era,
  title={Era of big data processing: A new approach via tensor networks and tensor decompositions},
  author={Cichocki, Andrzej},
  journal={arXiv preprint arXiv:1403.2048},
  year={2014}
}

@article{he2017wider,
  title={Wider and Deeper, Cheaper and Faster: Tensorized LSTMs for Sequence Learning},
  author={He, Zhen and Gao, Shaobing and Xiao, Liang and Liu, Daxue and He, Hangen and Barber, David},
  journal={arXiv preprint arXiv:1711.01577},
  year={2017}
}

@article{huang2016densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
  journal={arXiv preprint arXiv:1608.06993},
  year={2016}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{szegedy2017inception,
  title={Inception-v4, Inception-ResNet and the Impact of Residual Connections on Learning.},
  author={Szegedy, Christian and Ioffe, Sergey and Vanhoucke, Vincent and Alemi, Alexander A},
  booktitle={AAAI},
  pages={4278--4284},
  year={2017}
}

@inproceedings{han2015learning,
  title={Learning both weights and connections for efficient neural network},
  author={Han, Song and Pool, Jeff and Tran, John and Dally, William},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1135--1143},
  year={2015}
}

@inproceedings{byeon2015scene,
  title={Scene labeling with lstm recurrent neural networks},
  author={Byeon, Wonmin and Breuel, Thomas M and Raue, Federico and Liwicki, Marcus},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3547--3555},
  year={2015}
}

@inproceedings{liang2016semantic,
  title={Semantic object parsing with local-global long short-term memory},
  author={Liang, Xiaodan and Shen, Xiaohui and Xiang, Donglai and Feng, Jiashi and Lin, Liang and Yan, Shuicheng},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3185--3193},
  year={2016}
}

@inproceedings{theis2015generative,
  title={Generative image modeling using spatial LSTMs},
  author={Theis, Lucas and Bethge, Matthias},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1927--1935},
  year={2015}
}

@article{srivastava2014dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting.},
  author={Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={Journal of machine learning research},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014}
}


@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{wang2016blasx,
  title={Blasx: A high performance level-3 blas library for heterogeneous multi-gpu computing},
  author={Wang, Linnan and Wu, Wei and Xu, Zenglin and Xiao, Jianxiong and Yang, Yi},
  booktitle={Proceedings of the 2016 International Conference on Supercomputing},
  pages={20},
  year={2016},
  organization={ACM}
}

@article{wang2017accelerating,
  title={Accelerating deep neural network training with inconsistent stochastic gradient descent},
  author={Wang, Linnan and Yang, Yi and Min, Renqiang and Chakradhar, Srimat},
  journal={Neural Networks},
  year={2017},
  publisher={Elsevier}
}

@article{DBLP:journals/ftml/CichockiLOPZM16,
  author    = {Andrzej Cichocki and
               Namgil Lee and
               Ivan V. Oseledets and
               Anh Huy Phan and
               Qibin Zhao and
               Danilo P. Mandic},
  title     = {Tensor Networks for Dimensionality Reduction and Large-scale Optimization:
               Part 1 Low-Rank Tensor Decompositions},
  journal   = {Foundations and Trends in Machine Learning},
  volume    = {9},
  number    = {4-5},
  pages     = {249--429},
  year      = {2016},
  url       = {https://doi.org/10.1561/2200000059},
  doi       = {10.1561/2200000059},
  timestamp = {Sat, 20 May 2017 00:22:30 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/ftml/CichockiLOPZM16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/cvpr/DonahueHGRVDS15,
  author    = {Jeff Donahue and
               Lisa Anne Hendricks and
               Sergio Guadarrama and
               Marcus Rohrbach and
               Subhashini Venugopalan and
               Trevor Darrell and
               Kate Saenko},
  title     = {Long-term recurrent convolutional networks for visual recognition
               and description},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {2625--2634},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7298878},
  doi       = {10.1109/CVPR.2015.7298878},
  timestamp = {Thu, 15 Jun 2017 21:35:57 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/cvpr/DonahueHGRVDS15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/nips/DentonZBLF14,
  author    = {Emily L. Denton and
               Wojciech Zaremba and
               Joan Bruna and
               Yann LeCun and
               Rob Fergus},
  editor    = {Zoubin Ghahramani and
               Max Welling and
               Corinna Cortes and
               Neil D. Lawrence and
               Kilian Q. Weinberger},
  title     = {Exploiting Linear Structure Within Convolutional Networks for Efficient
               Evaluation},
  booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
               on Neural Information Processing Systems 2014, December 8-13 2014,
               Montreal, Quebec, Canada},
  pages     = {1269--1277},
  year      = {2014},
  url       = {http://papers.nips.cc/paper/5544-exploiting-linear-structure-within-convolutional-networks-for-efficient-evaluation},
  timestamp = {Wed, 10 Dec 2014 21:34:12 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/nips/DentonZBLF14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

